Tempus Core: Area-Power Efficient Temporal-Unary Convolution Core for Low-Precision Edge DLAs

The increasing complexity of deep neural networks (DNNs) poses significant challenges for edge inference deployment due to resource and power constraints of edge devices. Recent works on unary-based matrix multiplication hardware aim to leverage data sparsity and low-precision values to enhance hardware efficiency. However, the adoption and integration of such unary hardware into commercial deep learning accelerators (DLA) remain limited due to processing element (PE) array dataflow differences. This work presents Tempus Core, a convolution core with highly scalable unary-based PE array comprising of tub (temporal-unary-binary) multipliers that seamlessly integrates with the NVDLA (NVIDIA's open-source DLA for accelerating CNNs) while maintaining dataflow compliance and boosting hardware efficiency. Analysis across various datapath granularities shows that for INT8 precision in 45nm CMOS, Tempus Core's PE cell unit (PCU) yields 59.3% and 15.3% reductions in area and power consumption, respectively, over NVDLA's CMAC unit. Considering a 16x16 PE array in Tempus Core, area and power improves by 75% and 62%, respectively, while delivering 5x and 4x iso-area throughput improvements for INT8 and INT4 precisions. Post-place and route analysis of Tempus Core's PCU shows that the 16x4 PE array for INT4 precision in 45nm CMOS requires only 0.017 mm^2 die area and consumes only 6.2mW of total power. We demonstrate that area-power efficient unary-based hardware can be seamlessly integrated into conventional DLAs, paving the path for efficient unary hardware for edge AI inference.

==> NVDLA_TubGEMM_Integration.tex <==
To integrate TubGEMM into NVDLA, we need to first understand what the current mac unit in NVDLA is doing. The current mac unit inside NVDLA CMAC core is performing element-wise multiplication between the array of weights and array of feature values. It then takes the output array from the multiplication and sums up all the individual values into a single output value. This is a challenge for tubGEMM because tubGEMM performs A x B + C where A, B, and C are matrices and A x B is a normal matrix multiplication and not element-wise matrix multiplication.

\begin{figure}[!h]
    \centering
    \includegraphics[width=85mm]{images/tubGEMM-Based-CMAC_Arch.png}
    \caption{Architecture of tubGEMM-based CMAC}
    \label{fig:label}
\end{figure}

At first glance it might seem like the integration is incompatible, but with a clever math trick we could make tubGEMM perform the mac arithmetic needed for NVDLA. The trick is to transpose one of the two input arrays and then do normal matrix multiplication between the two arrays. This is possible because of two factors: 
\begin{itemize}
    \item the weight and feature matrix are always effectively 1-by-n matrices where n is the number of weights/features.
    \item $W \times F^T =$ accum($W \odot F$) where $W$ is the 1-by-$n$ matrix of weight values, $F$ is the 1-by-$n$ matrix of feature values, $n$ is the number of values in the matrix, and accum being the accumulation function.
\end{itemize}
The first is true because the weight and feature matrix are always effectively 1-by-n matrices where n is the number of weights/features. Element-wise matrix multiplication accumulate only cares that the corresponding weight and feature are in the same matrix location so the correct pairs are multiplied with each other since the shape of the matrix will ultimately be reduced down to a single value after accumulation.\\
The second is true because a matrix multiplication between a 1-by-n matrix and a n-by-1 matrix results in all the row values in the first matrix getting multiply by the corresponding column value of the second matrix and then summed together.\\
This means that the integration between NVDLA and TubGEMM is actually very easy since transposing in hardware is just flipping the row and column size parameter of the second matrix and the data structure itself doesn't need to change. The resulting integrated tubGEMM code is shown in figure 4. What is even more powerful about this integration is that it demonstrates that ANY GEMM accelerator can be used to accelerate the MAC operation desired by convolution-heavy workloads as well.
\begin{figure}[!h]
    \centering
    \includegraphics[width=85mm]{images/figure4.PNG}
    \caption{Code for tubGEMM integration into NVDLA}
    \label{fig:label}
\end{figure}
